Towards 1 Gbps/UE in Cellular Systems: Understanding Ultra-Dense Small Cell Deployments

Todays heterogeneous networks comprised of mostly macrocells and indoor small cells will not be able to meet the upcoming traffic demands. Indeed, it is forecasted that at least a 100x network capacity increase will be required to meet the traffic demands in 2020. As a result, vendors and operators are now looking at using every tool at hand to improve network capacity. In this epic campaign, three paradigms are noteworthy, i.e., network densification, the use of higher frequency bands and spectral efficiency enhancement techniques. This paper aims at bringing further common understanding and analysing the potential gains and limitations of these three paradigms, together with the impact of idle mode capabilities at the small cells as well as the user equipment density and distribution in outdoor scenarios. Special attention is paid to network densification and its implications when transitioning to ultra-dense small cell deployments. Simulation results show that network densification with an average inter site distance of 35 m can increase the cell- edge UE throughput by up to 48x, while the use of the 10GHz band with a 500MHz bandwidth can increase the network capacity up to 5x. The use of beamforming with up to 4 antennas per small cell base station lacks behind with cell-edge throughput gains of up to 1.49x. Our study also shows how network densifications reduces multi-user diversity, and thus proportional fair alike schedulers start losing their advantages with respect to round robin ones. The energy efficiency of these ultra-dense small cell deployments is also analysed, indicating the need for energy harvesting approaches to make these deployments energy- efficient. Finally, the top ten challenges to be addressed to bring ultra-dense small cell deployments to reality are also discussed.

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/f_dipoleArray_antennaPatterns.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{002}[cc][cc]{\matlabtextA $330^{\circ}$}%
\psfrag{003}[cc][cc]{\matlabtextA $300^{\circ}$}%
\psfrag{004}[cc][cc]{\matlabtextA $270^{\circ}$}%
\psfrag{005}[cc][cc]{\matlabtextA $240^{\circ}$}%
\psfrag{006}[cc][cc]{\matlabtextA $210^{\circ}$}%
\psfrag{007}[cc][cc]{\matlabtextA $180^{\circ}$}%
\psfrag{008}[cc][cc]{\matlabtextA $150^{\circ}$}%
\psfrag{009}[cc][cc]{\matlabtextA $120^{\circ}$}%
\psfrag{010}[cc][cc]{\matlabtextA $90^{\circ}$}%
\psfrag{011}[cc][cc]{\matlabtextA $60^{\circ}$}%
\psfrag{012}[cc][cc]{\matlabtextA $30^{\circ}$}%
\psfrag{013}[cc][cc]{\matlabtextA $0^{\circ}$}%
\psfrag{014}[cc][cc]{\matlabtextA $-30$ dB}%
\psfrag{015}[cc][cc]{\matlabtextA $-20$ dB}%
\psfrag{016}[cc][cc]{\matlabtextA $-10$ dB}%
\psfrag{017}[cc][cc]{\matlabtextA $0$ dB}%
%
\providecommand\matlabtextB{\color[rgb]{1.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextB vertical}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,1.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{001}[cl][cl]{\matlabtextC horizontal}%
%
%% </text>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/f_dipoleArray_spatialGain.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextA y[m]}%
\psfrag{022}[tc][tc]{\matlabtextA x[m]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{007}[ct][ct]{\matlabtextA $\matlabfragNegXTick 600$}%
\psfrag{008}[ct][ct]{\matlabtextA $\matlabfragNegXTick 400$}%
\psfrag{009}[ct][ct]{\matlabtextA $\matlabfragNegXTick 200$}%
\psfrag{010}[ct][ct]{\matlabtextA $0$}%
\psfrag{011}[ct][ct]{\matlabtextA $200$}%
\psfrag{012}[ct][ct]{\matlabtextA $400$}%
\psfrag{013}[ct][ct]{\matlabtextA $600$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextA $-40$}%
\psfrag{001}[lc][lc]{\matlabtextA $-30$}%
\psfrag{002}[lc][lc]{\matlabtextA $-20$}%
\psfrag{003}[lc][lc]{\matlabtextA $-10$}%
\psfrag{004}[lc][lc]{\matlabtextA $0$}%
\psfrag{005}[lc][lc]{\matlabtextA $10$}%
\psfrag{006}[lc][lc]{\matlabtextA $20$}%
\psfrag{014}[rc][rc]{\matlabtextA $-600$}%
\psfrag{015}[rc][rc]{\matlabtextA $-400$}%
\psfrag{016}[rc][rc]{\matlabtextA $-200$}%
\psfrag{017}[rc][rc]{\matlabtextA $0$}%
\psfrag{018}[rc][rc]{\matlabtextA $200$}%
\psfrag{019}[rc][rc]{\matlabtextA $400$}%
\psfrag{020}[rc][rc]{\matlabtextA $600$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-100-freq-2-smallcellOnOff-1-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{031}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB CDF}%
\psfrag{033}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{008}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-0-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA ISD=200, Idle mode=0}%
\psfrag{019}[cl][cl]{\matlabtextA ISD=150, Idle mode=0}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=100, Idle mode=0}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=075, Idle mode=0}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=050, Idle mode=0}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=035, Idle mode=0}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020, Idle mode=0}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=010, Idle mode=0}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=005, Idle mode=0}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB CDF}%
\psfrag{028}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-0-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{031}[bc][bc]{\matlabtextB CDF}%
\psfrag{032}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA ISD=200, Idle mode=1}%
\psfrag{019}[cl][cl]{\matlabtextA ISD=150, Idle mode=1}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=100, Idle mode=1}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=075, Idle mode=1}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=050, Idle mode=1}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=035, Idle mode=1}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020, Idle mode=1}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=010, Idle mode=1}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=005, Idle mode=1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB CDF}%
\psfrag{028}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-1-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{031}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB CDF}%
\psfrag{033}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{008}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-600-freq-2-smallcellOnOff-1-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{031}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB CDF}%
\psfrag{033}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{008}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_cellWithAtLeastaUE_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{025}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=200m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=150m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=100m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Average number of active cells per km^2}%
\psfrag{027}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{006}[ct][ct]{\matlabtextC $1$}%
\psfrag{007}[ct][ct]{\matlabtextC $1.2$}%
\psfrag{008}[ct][ct]{\matlabtextC $1.4$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.6$}%
\psfrag{010}[ct][ct]{\matlabtextC $1.8$}%
\psfrag{011}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $100$}%
\psfrag{014}[rc][rc]{\matlabtextC $200$}%
\psfrag{015}[rc][rc]{\matlabtextC $300$}%
\psfrag{016}[rc][rc]{\matlabtextC $400$}%
\psfrag{017}[rc][rc]{\matlabtextC $500$}%
\psfrag{018}[rc][rc]{\matlabtextC $600$}%
\psfrag{019}[rc][rc]{\matlabtextC $700$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_energyEfficiency_f_-ueDensity-300-ueDistribution-1-freq-2-smallcellOnOff-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA sleep=5, ant.=4}%
\psfrag{024}[cl][cl]{\matlabtextA sleep=5, ant.=1}%
\psfrag{025}[cl][cl]{\matlabtextA sleep=4, ant.=4}%
\psfrag{026}[cl][cl]{\matlabtextA sleep=4, ant.=1}%
\psfrag{027}[cl][cl]{\matlabtextA sleep=3, ant.=4}%
\psfrag{028}[cl][cl]{\matlabtextA sleep=3, ant.=1}%
\psfrag{029}[cl][cl]{\matlabtextA sleep=2, ant.=4}%
\psfrag{030}[cl][cl]{\matlabtextA sleep=2, ant.=1}%
\psfrag{031}[cl][cl]{\matlabtextA sleep=1, ant.=4}%
\psfrag{032}[cl][cl]{\matlabtextA sleep=1, ant.=1}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=200m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=150m}%
\psfrag{037}[bl][bl]{\matlabtextA ISD=100m}%
\psfrag{038}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{039}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{040}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{041}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{042}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{043}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{033}[bc][bc]{\matlabtextB Total network energy efficency [bps/W]}%
\psfrag{034}[tc][tc]{\matlabtextB Number of cells per km^2}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
\psfrag{006}[ct][ct]{\matlabtextC $1200$}%
\psfrag{007}[ct][ct]{\matlabtextC $1400$}%
\psfrag{008}[ct][ct]{\matlabtextC $1600$}%
\psfrag{009}[ct][ct]{\matlabtextC $1800$}%
\psfrag{010}[ct][ct]{\matlabtextC $2000$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{011}[bc][bc]{\matlabtextC $\times10^{6}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $2$}%
\psfrag{015}[rc][rc]{\matlabtextC $3$}%
\psfrag{016}[rc][rc]{\matlabtextC $4$}%
\psfrag{017}[rc][rc]{\matlabtextC $5$}%
\psfrag{018}[rc][rc]{\matlabtextC $6$}%
\psfrag{019}[rc][rc]{\matlabtextC $7$}%
\psfrag{020}[rc][rc]{\matlabtextC $8$}%
\psfrag{021}[rc][rc]{\matlabtextC $9$}%
\psfrag{022}[rc][rc]{\matlabtextC $10$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_powerNetwork_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=300, freq.=10}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, freq.=5}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, freq.=3.5}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=300, freq.=2}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Network Tx Power per km^2 [dBm/km^2]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $10$}%
\psfrag{013}[rc][rc]{\matlabtextC $20$}%
\psfrag{014}[rc][rc]{\matlabtextC $30$}%
\psfrag{015}[rc][rc]{\matlabtextC $40$}%
\psfrag{016}[rc][rc]{\matlabtextC $50$}%
\psfrag{017}[rc][rc]{\matlabtextC $60$}%
\psfrag{018}[rc][rc]{\matlabtextC $70$}%
\psfrag{019}[rc][rc]{\matlabtextC $80$}%
\psfrag{020}[rc][rc]{\matlabtextC $90$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_powerNetwork_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Network Tx Power per km^2 [dBm/km^2]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $10$}%
\psfrag{014}[rc][rc]{\matlabtextC $20$}%
\psfrag{015}[rc][rc]{\matlabtextC $30$}%
\psfrag{016}[rc][rc]{\matlabtextC $40$}%
\psfrag{017}[rc][rc]{\matlabtextC $50$}%
\psfrag{018}[rc][rc]{\matlabtextC $60$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_powerSector_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, freq.=10}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, freq.=5}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=300, freq.=3.5}%
\psfrag{025}[cl][cl]{\matlabtextA UE densit.=300, freq.=2}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Small cell Tx Power if ON [dBm]}%
\psfrag{027}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $-20$}%
\psfrag{013}[rc][rc]{\matlabtextC $-10$}%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $40$}%
\psfrag{019}[rc][rc]{\matlabtextC $50$}%
\psfrag{020}[rc][rc]{\matlabtextC $60$}%
\psfrag{021}[rc][rc]{\matlabtextC $70$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_powerSector_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{025}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Small cell Tx Power if ON [dBm]}%
\psfrag{027}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $-20$}%
\psfrag{013}[rc][rc]{\matlabtextC $-10$}%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $40$}%
\psfrag{019}[rc][rc]{\matlabtextC $50$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_throughputUEs_5tile_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA frequency = 10GHz}%
\psfrag{022}[cl][cl]{\matlabtextA frequency = 5GHz}%
\psfrag{023}[cl][cl]{\matlabtextA frequency = 3.5GHz}%
\psfrag{024}[cl][cl]{\matlabtextA frequency = 2GHz}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB 5%-tile UE throughput [bps]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{8}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $2$}%
\psfrag{015}[rc][rc]{\matlabtextC $4$}%
\psfrag{016}[rc][rc]{\matlabtextC $6$}%
\psfrag{017}[rc][rc]{\matlabtextC $8$}%
\psfrag{018}[rc][rc]{\matlabtextC $10$}%
\psfrag{019}[rc][rc]{\matlabtextC $12$}%
\psfrag{020}[rc][rc]{\matlabtextC $14$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_throughputUEs_5tile_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA freq.=10, antennas=4}%
\psfrag{024}[cl][cl]{\matlabtextA freq.=10, antennas=2}%
\psfrag{025}[cl][cl]{\matlabtextA freq.=10, antennas=1}%
\psfrag{026}[cl][cl]{\matlabtextA freq.=2, antennas=4}%
\psfrag{027}[cl][cl]{\matlabtextA freq.=2, antennas=2}%
\psfrag{028}[cl][cl]{\matlabtextA freq.=2, antennas=1}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{029}[bc][bc]{\matlabtextB 5%-tile UE throughput [bps]}%
\psfrag{030}[tc][tc]{\matlabtextB Number of cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{8}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $2$}%
\psfrag{015}[rc][rc]{\matlabtextC $4$}%
\psfrag{016}[rc][rc]{\matlabtextC $6$}%
\psfrag{017}[rc][rc]{\matlabtextC $8$}%
\psfrag{018}[rc][rc]{\matlabtextC $10$}%
\psfrag{019}[rc][rc]{\matlabtextC $12$}%
\psfrag{020}[rc][rc]{\matlabtextC $14$}%
\psfrag{021}[rc][rc]{\matlabtextC $16$}%
\psfrag{022}[rc][rc]{\matlabtextC $18$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_throughputUEs_average_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA frequency = 10GHz}%
\psfrag{022}[cl][cl]{\matlabtextA frequency = 5GHz}%
\psfrag{023}[cl][cl]{\matlabtextA frequency = 3.5GHz}%
\psfrag{024}[cl][cl]{\matlabtextA frequency = 2GHz}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Average UE throughput [bps]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{9}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{017}[rc][rc]{\matlabtextC $2$}%
\psfrag{018}[rc][rc]{\matlabtextC $2.5$}%
\psfrag{019}[rc][rc]{\matlabtextC $3$}%
\psfrag{020}[rc][rc]{\matlabtextC $3.5$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_throughputUEs_average_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA freq.=10, antennas=4}%
\psfrag{024}[cl][cl]{\matlabtextA freq.=10, antennas=2}%
\psfrag{025}[cl][cl]{\matlabtextA freq.=10, antennas=1}%
\psfrag{026}[cl][cl]{\matlabtextA freq.=2, antennas=4}%
\psfrag{027}[cl][cl]{\matlabtextA freq.=2, antennas=2}%
\psfrag{028}[cl][cl]{\matlabtextA freq.=2, antennas=1}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{029}[bc][bc]{\matlabtextB Average UE throughput [bps]}%
\psfrag{030}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{9}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{017}[rc][rc]{\matlabtextC $2$}%
\psfrag{018}[rc][rc]{\matlabtextC $2.5$}%
\psfrag{019}[rc][rc]{\matlabtextC $3$}%
\psfrag{020}[rc][rc]{\matlabtextC $3.5$}%
\psfrag{021}[rc][rc]{\matlabtextC $4$}%
\psfrag{022}[rc][rc]{\matlabtextC $4.5$}%
%
%% </ytick>

==> 2014 - IEEE Surveys and Tutorials - Ultra dense small cell deployments/figures/r_usersSector_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{018}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{019}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{026}[bl][bl]{\matlabtextA ISD=200m}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=150m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=100m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{024}[bc][bc]{\matlabtextB Average number of connected UEs per cell}%
\psfrag{025}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
\providecommand\matlabtextC{\color[rgb]{1.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextC 1 UE per cell}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $0$}%
\psfrag{001}[ct][ct]{\matlabtextD $200$}%
\psfrag{002}[ct][ct]{\matlabtextD $400$}%
\psfrag{003}[ct][ct]{\matlabtextD $600$}%
\psfrag{004}[ct][ct]{\matlabtextD $800$}%
\psfrag{005}[ct][ct]{\matlabtextD $1000$}%
\psfrag{006}[ct][ct]{\matlabtextD $1200$}%
\psfrag{007}[ct][ct]{\matlabtextD $1400$}%
\psfrag{008}[ct][ct]{\matlabtextD $1600$}%
\psfrag{009}[ct][ct]{\matlabtextD $1800$}%
\psfrag{010}[ct][ct]{\matlabtextD $2000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextD $0$}%
\psfrag{012}[rc][rc]{\matlabtextD $5$}%
\psfrag{013}[rc][rc]{\matlabtextD $10$}%
\psfrag{014}[rc][rc]{\matlabtextD $15$}%
\psfrag{015}[rc][rc]{\matlabtextD $20$}%
\psfrag{016}[rc][rc]{\matlabtextD $25$}%
%
%% </ytick>

==> figures/f_dipoleArray_antennaPatterns.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{002}[cc][cc]{\matlabtextA $330^{\circ}$}%
\psfrag{003}[cc][cc]{\matlabtextA $300^{\circ}$}%
\psfrag{004}[cc][cc]{\matlabtextA $270^{\circ}$}%
\psfrag{005}[cc][cc]{\matlabtextA $240^{\circ}$}%
\psfrag{006}[cc][cc]{\matlabtextA $210^{\circ}$}%
\psfrag{007}[cc][cc]{\matlabtextA $180^{\circ}$}%
\psfrag{008}[cc][cc]{\matlabtextA $150^{\circ}$}%
\psfrag{009}[cc][cc]{\matlabtextA $120^{\circ}$}%
\psfrag{010}[cc][cc]{\matlabtextA $90^{\circ}$}%
\psfrag{011}[cc][cc]{\matlabtextA $60^{\circ}$}%
\psfrag{012}[cc][cc]{\matlabtextA $30^{\circ}$}%
\psfrag{013}[cc][cc]{\matlabtextA $0^{\circ}$}%
\psfrag{014}[cc][cc]{\matlabtextA $-30$ dB}%
\psfrag{015}[cc][cc]{\matlabtextA $-20$ dB}%
\psfrag{016}[cc][cc]{\matlabtextA $-10$ dB}%
\psfrag{017}[cc][cc]{\matlabtextA $0$ dB}%
%
\providecommand\matlabtextB{\color[rgb]{1.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextB vertical}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,1.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{001}[cl][cl]{\matlabtextC horizontal}%
%
%% </text>

==> figures/f_dipoleArray_spatialGain.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextA y[m]}%
\psfrag{022}[tc][tc]{\matlabtextA x[m]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{007}[ct][ct]{\matlabtextA $\matlabfragNegXTick 600$}%
\psfrag{008}[ct][ct]{\matlabtextA $\matlabfragNegXTick 400$}%
\psfrag{009}[ct][ct]{\matlabtextA $\matlabfragNegXTick 200$}%
\psfrag{010}[ct][ct]{\matlabtextA $0$}%
\psfrag{011}[ct][ct]{\matlabtextA $200$}%
\psfrag{012}[ct][ct]{\matlabtextA $400$}%
\psfrag{013}[ct][ct]{\matlabtextA $600$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextA $-40$}%
\psfrag{001}[lc][lc]{\matlabtextA $-30$}%
\psfrag{002}[lc][lc]{\matlabtextA $-20$}%
\psfrag{003}[lc][lc]{\matlabtextA $-10$}%
\psfrag{004}[lc][lc]{\matlabtextA $0$}%
\psfrag{005}[lc][lc]{\matlabtextA $10$}%
\psfrag{006}[lc][lc]{\matlabtextA $20$}%
\psfrag{014}[rc][rc]{\matlabtextA $-600$}%
\psfrag{015}[rc][rc]{\matlabtextA $-400$}%
\psfrag{016}[rc][rc]{\matlabtextA $-200$}%
\psfrag{017}[rc][rc]{\matlabtextA $0$}%
\psfrag{018}[rc][rc]{\matlabtextA $200$}%
\psfrag{019}[rc][rc]{\matlabtextA $400$}%
\psfrag{020}[rc][rc]{\matlabtextA $600$}%
%
%% </ytick>

==> figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-100-freq-2-smallcellOnOff-1-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{031}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB CDF}%
\psfrag{033}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{008}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-0-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA ISD=200, Idle mode=0}%
\psfrag{019}[cl][cl]{\matlabtextA ISD=150, Idle mode=0}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=100, Idle mode=0}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=075, Idle mode=0}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=050, Idle mode=0}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=035, Idle mode=0}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020, Idle mode=0}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=010, Idle mode=0}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=005, Idle mode=0}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB CDF}%
\psfrag{028}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-0-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{031}[bc][bc]{\matlabtextB CDF}%
\psfrag{032}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $50$}%
\psfrag{005}[ct][ct]{\matlabtextC $60$}%
\psfrag{006}[ct][ct]{\matlabtextC $70$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA ISD=200, Idle mode=1}%
\psfrag{019}[cl][cl]{\matlabtextA ISD=150, Idle mode=1}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=100, Idle mode=1}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=075, Idle mode=1}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=050, Idle mode=1}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=035, Idle mode=1}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020, Idle mode=1}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=010, Idle mode=1}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=005, Idle mode=1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB CDF}%
\psfrag{028}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-300-freq-2-smallcellOnOff-1-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{031}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB CDF}%
\psfrag{033}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{008}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/r_cdf_controlChannelSinrUEs_f_-ueDensity-600-freq-2-smallcellOnOff-1-smallCellAnts-transition-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA ISD=035,snrTarget=15}%
\psfrag{021}[cl][cl]{\matlabtextA ISD=035,snrTarget=12}%
\psfrag{022}[cl][cl]{\matlabtextA ISD=035,snrTarget=09}%
\psfrag{023}[cl][cl]{\matlabtextA ISD=020,snrTarget=15}%
\psfrag{024}[cl][cl]{\matlabtextA ISD=020,snrTarget=12}%
\psfrag{025}[cl][cl]{\matlabtextA ISD=020,snrTarget=09}%
\psfrag{026}[cl][cl]{\matlabtextA ISD=010,snrTarget=15}%
\psfrag{027}[cl][cl]{\matlabtextA ISD=010,snrTarget=12}%
\psfrag{028}[cl][cl]{\matlabtextA ISD=010,snrTarget=09}%
\psfrag{029}[cl][cl]{\matlabtextA ISD=005,snrTarget=15}%
\psfrag{030}[cl][cl]{\matlabtextA ISD=005,snrTarget=12}%
\psfrag{031}[cl][cl]{\matlabtextA ISD=005,snrTarget=09}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB CDF}%
\psfrag{033}[tc][tc]{\matlabtextB UE wideband SINR [dB]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{008}[ct][ct]{\matlabtextC $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> figures/r_cellWithAtLeastaUE_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{025}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=200m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=150m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=100m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Average number of active cells per km^2}%
\psfrag{027}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{006}[ct][ct]{\matlabtextC $1$}%
\psfrag{007}[ct][ct]{\matlabtextC $1.2$}%
\psfrag{008}[ct][ct]{\matlabtextC $1.4$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.6$}%
\psfrag{010}[ct][ct]{\matlabtextC $1.8$}%
\psfrag{011}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $100$}%
\psfrag{014}[rc][rc]{\matlabtextC $200$}%
\psfrag{015}[rc][rc]{\matlabtextC $300$}%
\psfrag{016}[rc][rc]{\matlabtextC $400$}%
\psfrag{017}[rc][rc]{\matlabtextC $500$}%
\psfrag{018}[rc][rc]{\matlabtextC $600$}%
\psfrag{019}[rc][rc]{\matlabtextC $700$}%
%
%% </ytick>

==> figures/r_energyEfficiency_f_-ueDensity-300-ueDistribution-1-freq-2-smallcellOnOff-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA sleep=5, ant.=4}%
\psfrag{024}[cl][cl]{\matlabtextA sleep=5, ant.=1}%
\psfrag{025}[cl][cl]{\matlabtextA sleep=4, ant.=4}%
\psfrag{026}[cl][cl]{\matlabtextA sleep=4, ant.=1}%
\psfrag{027}[cl][cl]{\matlabtextA sleep=3, ant.=4}%
\psfrag{028}[cl][cl]{\matlabtextA sleep=3, ant.=1}%
\psfrag{029}[cl][cl]{\matlabtextA sleep=2, ant.=4}%
\psfrag{030}[cl][cl]{\matlabtextA sleep=2, ant.=1}%
\psfrag{031}[cl][cl]{\matlabtextA sleep=1, ant.=4}%
\psfrag{032}[cl][cl]{\matlabtextA sleep=1, ant.=1}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=200m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=150m}%
\psfrag{037}[bl][bl]{\matlabtextA ISD=100m}%
\psfrag{038}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{039}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{040}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{041}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{042}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{043}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{033}[bc][bc]{\matlabtextB Total network energy efficency [bps/W]}%
\psfrag{034}[tc][tc]{\matlabtextB Number of cells per km^2}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
\psfrag{006}[ct][ct]{\matlabtextC $1200$}%
\psfrag{007}[ct][ct]{\matlabtextC $1400$}%
\psfrag{008}[ct][ct]{\matlabtextC $1600$}%
\psfrag{009}[ct][ct]{\matlabtextC $1800$}%
\psfrag{010}[ct][ct]{\matlabtextC $2000$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{011}[bc][bc]{\matlabtextC $\times10^{6}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $2$}%
\psfrag{015}[rc][rc]{\matlabtextC $3$}%
\psfrag{016}[rc][rc]{\matlabtextC $4$}%
\psfrag{017}[rc][rc]{\matlabtextC $5$}%
\psfrag{018}[rc][rc]{\matlabtextC $6$}%
\psfrag{019}[rc][rc]{\matlabtextC $7$}%
\psfrag{020}[rc][rc]{\matlabtextC $8$}%
\psfrag{021}[rc][rc]{\matlabtextC $9$}%
\psfrag{022}[rc][rc]{\matlabtextC $10$}%
%
%% </ytick>

==> figures/r_powerNetwork_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=300, freq.=10}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, freq.=5}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, freq.=3.5}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=300, freq.=2}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Network Tx Power per km^2 [dBm/km^2]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $10$}%
\psfrag{013}[rc][rc]{\matlabtextC $20$}%
\psfrag{014}[rc][rc]{\matlabtextC $30$}%
\psfrag{015}[rc][rc]{\matlabtextC $40$}%
\psfrag{016}[rc][rc]{\matlabtextC $50$}%
\psfrag{017}[rc][rc]{\matlabtextC $60$}%
\psfrag{018}[rc][rc]{\matlabtextC $70$}%
\psfrag{019}[rc][rc]{\matlabtextC $80$}%
\psfrag{020}[rc][rc]{\matlabtextC $90$}%
%
%% </ytick>

==> figures/r_powerNetwork_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Network Tx Power per km^2 [dBm/km^2]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $10$}%
\psfrag{014}[rc][rc]{\matlabtextC $20$}%
\psfrag{015}[rc][rc]{\matlabtextC $30$}%
\psfrag{016}[rc][rc]{\matlabtextC $40$}%
\psfrag{017}[rc][rc]{\matlabtextC $50$}%
\psfrag{018}[rc][rc]{\matlabtextC $60$}%
%
%% </ytick>

==> figures/r_powerSector_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, freq.=10}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, freq.=5}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=300, freq.=3.5}%
\psfrag{025}[cl][cl]{\matlabtextA UE densit.=300, freq.=2}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Small cell Tx Power if ON [dBm]}%
\psfrag{027}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $-20$}%
\psfrag{013}[rc][rc]{\matlabtextC $-10$}%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $40$}%
\psfrag{019}[rc][rc]{\matlabtextC $50$}%
\psfrag{020}[rc][rc]{\matlabtextC $60$}%
\psfrag{021}[rc][rc]{\matlabtextC $70$}%
%
%% </ytick>

==> figures/r_powerSector_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{023}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{024}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{025}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB Small cell Tx Power if ON [dBm]}%
\psfrag{027}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $-20$}%
\psfrag{013}[rc][rc]{\matlabtextC $-10$}%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $40$}%
\psfrag{019}[rc][rc]{\matlabtextC $50$}%
%
%% </ytick>

==> figures/r_throughputUEs_5tile_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA frequency = 10GHz}%
\psfrag{022}[cl][cl]{\matlabtextA frequency = 5GHz}%
\psfrag{023}[cl][cl]{\matlabtextA frequency = 3.5GHz}%
\psfrag{024}[cl][cl]{\matlabtextA frequency = 2GHz}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB 5%-tile UE throughput [bps]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{8}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $2$}%
\psfrag{015}[rc][rc]{\matlabtextC $4$}%
\psfrag{016}[rc][rc]{\matlabtextC $6$}%
\psfrag{017}[rc][rc]{\matlabtextC $8$}%
\psfrag{018}[rc][rc]{\matlabtextC $10$}%
\psfrag{019}[rc][rc]{\matlabtextC $12$}%
\psfrag{020}[rc][rc]{\matlabtextC $14$}%
%
%% </ytick>

==> figures/r_throughputUEs_5tile_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA freq.=10, antennas=4}%
\psfrag{024}[cl][cl]{\matlabtextA freq.=10, antennas=2}%
\psfrag{025}[cl][cl]{\matlabtextA freq.=10, antennas=1}%
\psfrag{026}[cl][cl]{\matlabtextA freq.=2, antennas=4}%
\psfrag{027}[cl][cl]{\matlabtextA freq.=2, antennas=2}%
\psfrag{028}[cl][cl]{\matlabtextA freq.=2, antennas=1}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{029}[bc][bc]{\matlabtextB 5%-tile UE throughput [bps]}%
\psfrag{030}[tc][tc]{\matlabtextB Number of cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{8}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $2$}%
\psfrag{015}[rc][rc]{\matlabtextC $4$}%
\psfrag{016}[rc][rc]{\matlabtextC $6$}%
\psfrag{017}[rc][rc]{\matlabtextC $8$}%
\psfrag{018}[rc][rc]{\matlabtextC $10$}%
\psfrag{019}[rc][rc]{\matlabtextC $12$}%
\psfrag{020}[rc][rc]{\matlabtextC $14$}%
\psfrag{021}[rc][rc]{\matlabtextC $16$}%
\psfrag{022}[rc][rc]{\matlabtextC $18$}%
%
%% </ytick>

==> figures/r_throughputUEs_average_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA frequency = 10GHz}%
\psfrag{022}[cl][cl]{\matlabtextA frequency = 5GHz}%
\psfrag{023}[cl][cl]{\matlabtextA frequency = 3.5GHz}%
\psfrag{024}[cl][cl]{\matlabtextA frequency = 2GHz}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB Average UE throughput [bps]}%
\psfrag{026}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{9}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{017}[rc][rc]{\matlabtextC $2$}%
\psfrag{018}[rc][rc]{\matlabtextC $2.5$}%
\psfrag{019}[rc][rc]{\matlabtextC $3$}%
\psfrag{020}[rc][rc]{\matlabtextC $3.5$}%
%
%% </ytick>

==> figures/r_throughputUEs_average_f_-ueDensity-300-ueDistribution-1-smallcellOnOff-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA freq.=10, antennas=4}%
\psfrag{024}[cl][cl]{\matlabtextA freq.=10, antennas=2}%
\psfrag{025}[cl][cl]{\matlabtextA freq.=10, antennas=1}%
\psfrag{026}[cl][cl]{\matlabtextA freq.=2, antennas=4}%
\psfrag{027}[cl][cl]{\matlabtextA freq.=2, antennas=2}%
\psfrag{028}[cl][cl]{\matlabtextA freq.=2, antennas=1}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{035}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{036}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{029}[bc][bc]{\matlabtextB Average UE throughput [bps]}%
\psfrag{030}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[tc][tc]{\matlabtextC $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $2$}%
\psfrag{006}[ct][ct]{\matlabtextC $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $3.5$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $4.5$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{012}[bc][bc]{\matlabtextC $\times10^{9}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{017}[rc][rc]{\matlabtextC $2$}%
\psfrag{018}[rc][rc]{\matlabtextC $2.5$}%
\psfrag{019}[rc][rc]{\matlabtextC $3$}%
\psfrag{020}[rc][rc]{\matlabtextC $3.5$}%
\psfrag{021}[rc][rc]{\matlabtextC $4$}%
\psfrag{022}[rc][rc]{\matlabtextC $4.5$}%
%
%% </ytick>

==> figures/r_usersSector_f_freq-2-smallcellOnOff-1-smallCellAnts-1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=1}%
\psfrag{018}[cl][cl]{\matlabtextA UE densit.=600, UE distr.=0}%
\psfrag{019}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=1}%
\psfrag{020}[cl][cl]{\matlabtextA UE densit.=300, UE distr.=0}%
\psfrag{021}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=1}%
\psfrag{022}[cl][cl]{\matlabtextA UE densit.=100, UE distr.=0}%
\psfrag{026}[bl][bl]{\matlabtextA ISD=200m}%
\psfrag{027}[bl][bl]{\matlabtextA ISD=150m}%
\psfrag{028}[bl][bl]{\matlabtextA ISD=100m}%
\psfrag{029}[bl][bl]{\matlabtextA ISD=75m}%
\psfrag{030}[bl][bl]{\matlabtextA ISD=50m}%
\psfrag{031}[bl][bl]{\matlabtextA ISD=35m}%
\psfrag{032}[bl][bl]{\matlabtextA ISD=20m}%
\psfrag{033}[bl][bl]{\matlabtextA ISD=10m}%
\psfrag{034}[bl][bl]{\matlabtextA ISD=5m}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{024}[bc][bc]{\matlabtextB Average number of connected UEs per cell}%
\psfrag{025}[tc][tc]{\matlabtextB Number of small cells per km^2}%
%
\providecommand\matlabtextC{\color[rgb]{1.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextC 1 UE per cell}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $0$}%
\psfrag{001}[ct][ct]{\matlabtextD $200$}%
\psfrag{002}[ct][ct]{\matlabtextD $400$}%
\psfrag{003}[ct][ct]{\matlabtextD $600$}%
\psfrag{004}[ct][ct]{\matlabtextD $800$}%
\psfrag{005}[ct][ct]{\matlabtextD $1000$}%
\psfrag{006}[ct][ct]{\matlabtextD $1200$}%
\psfrag{007}[ct][ct]{\matlabtextD $1400$}%
\psfrag{008}[ct][ct]{\matlabtextD $1600$}%
\psfrag{009}[ct][ct]{\matlabtextD $1800$}%
\psfrag{010}[ct][ct]{\matlabtextD $2000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextD $0$}%
\psfrag{012}[rc][rc]{\matlabtextD $5$}%
\psfrag{013}[rc][rc]{\matlabtextD $10$}%
\psfrag{014}[rc][rc]{\matlabtextD $15$}%
\psfrag{015}[rc][rc]{\matlabtextD $20$}%
\psfrag{016}[rc][rc]{\matlabtextD $25$}%
%
%% </ytick>
